Every Component Counts: Rethinking the Measure of Success for Medical Semantic Segmentation in Multi-Instance Segmentation Tasks

We present Connected-Component~(CC)-Metrics, a novel semantic segmentation evaluation protocol, targeted to align existing semantic segmentation metrics to a multi-instance detection scenario in which each connected component matters. We motivate this setup in the common medical scenario of semantic metastases segmentation in a full-body PET/CT. We show how existing semantic segmentation metrics suffer from a bias towards larger connected components contradicting the clinical assessment of scans in which tumor size and clinical relevance are uncorrelated. To rebalance existing segmentation metrics, we propose to evaluate them on a per-component basis thus giving each tumor the same weight irrespective of its size. To match predictions to ground-truth segments, we employ a proximity-based matching criterion, evaluating common metrics locally at the component of interest. Using this approach, we break free of biases introduced by large metastasis for overlap-based metrics such as Dice or Surface Dice. CC-Metrics also improves distance-based metrics such as Hausdorff Distances which are uninformative for small changes that do not influence the maximum or 95th percentile, and avoids pitfalls introduced by directly combining counting-based metrics with overlap-based metrics as it is done in Panoptic Quality.

==> Latex/reproducability_checklist.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: Yes
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: Yes
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: Yes
\end{itemize}

Does this paper make theoretical contributions: No

Does this paper rely on one or more datasets: Yes
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets: Yes
    \item All novel datasets introduced in this paper are included in a data appendix: N/A
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: N/A
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations: Yes
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available: Yes
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing: N/A
\end{itemize}

Does this paper include computational experiments: Yes

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix: Yes
    \item All source code required for conducting and analyzing the experiments is included in a code appendix: Yes
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: Yes
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from: Partial
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results: Partial
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks: Yes
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics: Yes
    \item This paper states the number of algorithm runs used to compute each reported result: Yes
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information: Yes
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank): No, not applicable 
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments: Yes
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting: Yes
\end{itemize}
